Semi-Supervised State-Space Model with Dynamic Stacking Filter for Real-World Video Deraining

Significant progress has been made in video restoration under rainy conditions over the past decade, largely propelled by advancements in deep learning. Nevertheless, existing methods that depend on paired data struggle to generalize effectively to real-world scenarios, primarily due to the disparity between synthetic and authentic rain effects. To address these limitations, we propose a dual-branch spatio-temporal state-space model to enhance rain streak removal in video sequences. Specifically, we design spatial and temporal state-space model layers to extract spatial features and incorporate temporal dependencies across frames, respectively. To improve multi-frame feature fusion, we derive a dynamic stacking filter, which adaptively approximates statistical filters for superior pixel-wise feature refinement. Moreover, we develop a median stacking loss to enable semi-supervised learning by generating pseudo-clean patches based on the sparsity prior of rain. To further explore the capacity of deraining models in supporting other vision-based tasks in rainy environments, we introduce a novel real-world benchmark focused on object detection and tracking in rainy conditions. Our method is extensively evaluated across multiple benchmarks containing numerous synthetic and real-world rainy videos, consistently demonstrating its superiority in quantitative metrics, visual quality, efficiency, and its utility for downstream tasks.

==> sec/ackno.tex <==
\section*{Acknowledgments}
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.


==> sec/algor.tex <==
\begin{algorithm}[H]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{The training and inference pipeline of RTRWNet.}\label{alg:alg1}
\begin{algorithmic}[1]
\REQUIRE {pre-trained pair-wise optical flow estimation teacher $\mathcal{T}$, multi-frame optical flow estimator $\mathcal{S}$, paired rainy dataset $\mathcal{D}^{pair}=\{\{I_i\}_{i=t-d}^{t+d}, \{B_i\}_{i=t-d}^{t+d}\}$, unpaired rainy dataset $\mathcal{D}^{unpair}=\{\{I_i\}_{i=t-d}^{t+d}\}$, }
\ENSURE {RTRWNet consisting of a distilled multi-flow estimator $\mathcal{S}$ and a trained deraining network $\mathcal{F}$}
\STATE {\textsc{Multi-frame optical flow Distillation}}
\FOR{$\{I_i\}_{i=t-d}^{t+d}, \{B_i\}_{i=t-d}^{t+d} \in \mathcal{D}^{pair}$}
\STATE optimize $\mathcal{S}$ by minimizing $\mathcal{L}_{distillation}$ in Eq.~\ref{eq:distillation_loss} ;
\ENDFOR
% \STATE 
\STATE {\textsc{Deraining Training}}
\FOR{$x \in \mathcal{D}^{pair}\bigcup \mathcal{D}^{unpair}$}
\IF{$x\in \mathcal{D}^{pair}$} 
\STATE compute $\mathcal{L}\gets \lambda_1\mathcal{L}_{reconstruction}$ in Eq.~\ref{eq:reconstruction_loss}
\ELSE[$x\in \mathcal{D}^{unpair}$]
\STATE compute $\mathcal{L}\gets \lambda_2\mathcal{L}_{stacking}$ in Eq.~\ref{eq:stacking_loss}
\ENDIF 
\STATE compute $\mathcal{L}_{temporal}$ in Eq.~\ref{eq:temporal_loss}
\STATE optimize $\mathcal{F}$ by minimizing $\mathcal{L} + \lambda_3 \mathcal{L}_{temporal}$
\ENDFOR
% \STATE 
\STATE {\textsc{INFERENCE}}
\STATE estimate multi-frame optical flow and warp the neighbor frames by Eq.~\ref{eq:warped_frames}
\STATE predict deraining result by Eq.~\ref{eq:deraining_result}
\end{algorithmic}
\label{alg1}
\end{algorithm}

==> sec/appen.tex <==
{\appendix[Proof of the Zonklar Equations]
Use $\backslash${\tt{appendix}} if you have a single appendix:
Do not use $\backslash${\tt{section}} anymore after $\backslash${\tt{appendix}}, only $\backslash${\tt{section*}}.
If you have multiple appendixes use $\backslash${\tt{appendices}} then use $\backslash${\tt{section}} to start each appendix.
You must declare a $\backslash${\tt{section}} before using any $\backslash${\tt{subsection}} or using $\backslash${\tt{label}} ($\backslash${\tt{appendices}} by itself
 starts a section numbered zero.)}


==> sec/biogr.tex <==

% %-------------------------------------------------------------------------
% \newpage
% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}


\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,trim={0 0.5cm 0 1.7cm},clip,keepaspectratio]{fig/biography/shangquan.JPG}}]{Shangquan Sun}
is currently a Ph.D. candidate at the Institute of Information Engineering, Chinese Academy of Sciences, Beijing, China, and the School of Cyber Security, University of Chinese Academy of Sciences, Beijing, China. His research interests include low-level image processing.
\end{IEEEbiography}

\vspace{-10.5mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/biography/wenqi.png}}]{Wenqi Ren}
(Member, IEEE) received the Ph.D. degree from Tianjin University, Tianjin, China, in 2017. From 2015 to 2016, he was supported by the China Scholarship Council and working with Prof. Ming-Husan Yang as a joint-training Ph.D. Student with the Electrical Engineering and Computer Science Department, University of California at Merced. He is currently an Associate Professor with the School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University, Shenzhen, China. His research interests include image processing and related high-level vision problems.
\end{IEEEbiography}

\vspace{-10.5mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/biography/rui.jpeg}}]{Rui Wang}
(Member, IEEE) received the bachelor's degree from Tsinghua University, China, in 2005, and the Ph.D. degree from Graduate University of Chinese Academy of Sciences, China, in 2011. Currently, she works in Institute of Information Engineering, Chinese Academy of Sciences, as a professor and doctoral supervisor. Her research interests include computer vision and artificial intelligence security..
\end{IEEEbiography}

\vspace{-10.5mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/biography/xiaochun.png}}]{Xiaochun Cao}
(Senior Member, IEEE) is a Professor and Dean of School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University. He received the B.E. and M.E. degrees both in computer science from Beihang University (BUAA), China, and the Ph.D. degree in computer science from the University of Central Florida, USA, with his dissertation nominated for the university level Outstanding Dissertation Award. After graduation, he spent about three years at ObjectVideo Inc. as a Research Scientist. From 2008 to 2012, he was a professor at Tianjin University. Before joining SYSU, he was a professor at Institute of Information Engineering, Chinese Academy of Sciences. He has authored and coauthored over 200 journal and conference papers. In 2004 and 2010, he was the recipients of the Piero Zamperoni best student paper award at the International Conference on Pattern Recognition. He is on the editorial boards of IEEE Transactions on Pattern Analysis and Machine Intelligence and IEEE Transactions on Image Processing, and was on the editorial boards of IEEE Transactions on Circuits and Systems for Video Technology and IEEE Transactions on Multimedia.  
\end{IEEEbiography}

\vspace{-10.5mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/biography/wei.png}}]{Wei Liu} 
(M’14-SM’19-F’23) received the Ph.D. degree from Columbia University in 2012 in Electrical Engineering and Computer Science. He is currently a Distinguished Scientist of Tencent and the Director of Ads Multimedia AI at Tencent Data Platform. Prior to that, he has been a research staff member of IBM T. J. Watson Research Center, USA from 2012 to 2015. Dr. Liu has long been devoted to fundamental research
and technological development in core fields of AI, including deep learning, machine learning, reinforcement learning, computer vision, information retrieval, big data, etc. To date, he has published extensively in these fields with more than 280 peer-reviewed technical papers, and also issued over 30 US patents. He currently serves on the editorial boards of internationally leading AI journals like IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI), IEEE Transactions on Neural Networks and Learning Systems (TNNLS), and IEEE Intelligent Systems. He is an Area Chair of top-tier computer science and AI conferences, e.g., NeurIPS, ICML, IEEE CVPR, IEEE ICCV, IJCAI, and AAAI. Dr. Liu is a Fellow of the IEEE, IAPR, and IMA, and an Elected Member of the ISI..
\end{IEEEbiography}
% \vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}

% %-------------------------------------------------------------------------

==> sec/refer.tex <==
{\small
\bibliographystyle{IEEEtran}
\bibliography{pami/ref}
}


==> sec_fig/complexities.tex <==

\begin{figure}[t]
  \centering
  \subfloat[Time Complexity]{\label{fig:complexities-time}\includegraphics[width=0.49\linewidth]{fig/complexities/plot_time_complxty1.pdf}}
  \hfill
  \subfloat[Space Complexity]{\label{fig:complexities-space}\includegraphics[width=0.49\linewidth]{fig/complexities/plot_space_complxty1.pdf}}
% \setlength{\abovecaptionskip}{-0.1pt} 
% \setlength{\belowcaptionskip}{-17pt}
  \caption{The time and space complexities of the compared deraining methods. The red line in \ref{fig:complexities-time} denotes the boundary of real-time inference.}
  \label{fig:complexities}
  \vspace{-5mm}
\end{figure}

==> sec_fig/distillation.tex <==

\begin{figure}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1\linewidth]{fig/arch/multiframe_distillation2.pdf}
\setlength{\abovecaptionskip}{-15pt} 
\setlength{\belowcaptionskip}{-15pt}
   \caption{The pipeline of degradation-free multi-frame optical flow distillation. }
   \label{fig:multiframe_distillation}
   \vspace{-3mm}
\end{figure}

==> sec_fig/fig_rebuttal.tex <==

\begin{figure}[t]
  \centering
  \centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_Rainy_00137.jpg}
  \hspace{-1.5mm}
  \centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_S2VD_00135.png}
  \hspace{-1.5mm}
  \centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_Ours_00137.png}

  % \vspace{-3mm}
  \centering
  \subfloat[Rainy]{\label{fig:fig_rebuttal-rainy}\centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_Rainy_00011.png}}
  \hfill
  \subfloat[S2VD]{\label{fig:fig_rebuttal-s2vd}\centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_S2VD_00011.png}}
  \hfill
  \subfloat[Ours]{\label{fig:fig_rebuttal-ours}\centering\includegraphics[width=0.331\linewidth]{fig/result/rebuttal/ra1/ra1_Ours_00011.png}}
\vspace{-3.5mm}
  \caption{Additional Commparisons against S2VD on NTURain.}
  \label{fig:fig_rebuttal}
  \vspace{-4mm}
\end{figure}

==> sec_fig/limitation.tex <==

\begin{figure}[t]
  \centering
  \subfloat[Rainy $I_t$]{\label{fig:warp_example-rainy1}\includegraphics[trim=0 {0.3\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/rect_croped_4_5_target.jpg}}
  \hfill
  \subfloat[Flow by $\mathcal{T}$]{\label{fig:warp_example-flow1}\includegraphics[trim=0 {0.43\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/crop_flow3.png}}
  \hfill
  \subfloat[Warped by (b)]{\label{fig:warp_example-warp1}\includegraphics[trim=0 {0.3\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/rect_warped_multiframe_3.png}}

  
  \vspace{-3mm}
  \centering
  \subfloat[Rainy $I_{t+1}$]{\label{fig:warp_example-rainy2}\includegraphics[trim=0 {0.3\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/rect_croped_5_5_target.jpg}}
  \hfill
  \subfloat[Flow by ours]{\label{fig:warp_example-flow2}\includegraphics[trim=0 {0.43\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/crop_flow_gt3.png}}
  \hfill
  \subfloat[Warped by (e)]{\label{fig:warp_example-warp2}\includegraphics[trim=0 {0.3\linewidth} 0 0,clip,width=0.33\linewidth]{fig/warp_example/rect_warped_multiframe_gt_3.png}}
\setlength{\abovecaptionskip}{-0.1pt} 
\setlength{\belowcaptionskip}{-17pt}
  \caption{.}
  \label{fig:warp_example}
  \vspace{-3mm}
\end{figure}

==> sec_fig/result/nturain_syn.tex <==
\begin{figure*}[t]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:nturain_syn-a}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/rainy/00137.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:nturain_syn-b}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/fastderain/0137.jpg}}
  \hfill
  \subfloat[SLDNet~\cite{Yang2020Self} \label{fig:nturain_syn-c}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/sldnet/00137_res.png}}
  \hfill
  \subfloat[S2VD~\cite{Yue2021Semi} \label{fig:nturain_syn-d}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/s2vd/00135.png}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:nturain_syn-e}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/estinet/1568_0_2.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:nturain_syn-f}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/mfgan/00137_s2.png}}
  \hfill
  \subfloat[Ours\label{fig:nturain_syn-g}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/ours/00137.png}}
  \hfill
  \subfloat[Clean\label{fig:nturain_syn-h}]{\includegraphics[width=0.245\linewidth]{fig/result/nturain_syn/gt/00137.jpg}}
  
    
\setlength{\abovecaptionskip}{2pt} 
\setlength{\belowcaptionskip}{-1pt}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a synthetic rainy video with fast moving backgrounds from NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:nturain_syn}
  % \vspace{-0.5cm}
\end{figure*}

==> sec_fig/result/ra2.tex <==
\begin{figure*}[t]
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00049.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0049.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/fastderain/0049.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/spaccnn/00049.jpg}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00063.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0063.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/fastderain/0063.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/spaccnn/00063.jpg}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00064.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0064.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/fastderain/0064.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/spaccnn/00064.jpg}
  
  \vspace{-2.5mm}
  \centering
  \subfloat[Rainy\label{fig:realra2-a}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00065.jpg}}
  \hfill
  \subfloat[MSCSC~\cite{Li2018VideoRainStreak} \label{fig:realra2-b}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0065.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:realra2-c}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/fastderain/0065.jpg}}
  \hfill
  \subfloat[SpacCNN\label{fig:realra2-c}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/spaccnn/00065.jpg}}
  
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00063.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00063.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00063_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00063.png}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00064.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00064.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00064_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00064.png}
  
  \vspace{-2.5mm}
  \centering
  \subfloat[S2VD~\cite{Yue2021Semi}\label{fig:realra2-e}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00065.png}}
  \hfill
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:realra2-f}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00065.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:realra2-g}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00065_s2.png}}
  \hfill
  \subfloat[Ours\label{fig:realra2-h}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00065.png}}
  
    
% \setlength{\abovecaptionskip}{1pt} 
% \setlength{\belowcaptionskip}{-10pt}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a real-world rainy video from NTURain~\cite{Chen2018RobustCNN}. }
  \label{fig:real2}
  % \vspace{-0.4cm}
\end{figure*}

==> sec_fig/result/ra2_horizontal.tex <==
\newpage
\begin{figure*}[!hp]
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00049.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00063.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00064.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/rainy/00065.jpg}
  
  % \vspace{1mm}
  % \centering
  % \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0049.jpg}
  % \hfill
  % \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0063.jpg}
  % \hfill
  % \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0064.jpg}
  % \hfill
  % \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mscsc/0065.jpg}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/drsformer/00049.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/drsformer/00063.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/drsformer/00064.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/drsformer/00065.png}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00049.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00063.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00064.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/s2vd/00065.png}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00049.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00063.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00064.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/estinet/00065.png}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00049_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00063_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00064_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/mfgan/00065_s2.png}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/sldnet/00049_res.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/sldnet/00063_res.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/sldnet/00064_res.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra2/sldnet/00065_res.png}
  
  \vspace{-2.5mm}
  \centering
  \subfloat[Frame 1\label{fig:realra2-a}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00049.png}}
  \hfill
  \subfloat[Frame 2\label{fig:realra2-b}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00063.png}}
  \hfill
  \subfloat[Frame 3\label{fig:realra2-c}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00064.png}}
  \hfill
  \subfloat[Frame 4\label{fig:realra2-d}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra2/ours/00065.png}}
  
    
% \setlength{\abovecaptionskip}{1pt} 
% \setlength{\belowcaptionskip}{-10pt}
  \caption{The visual comparison among the state-of-the-art deraining methods on four consecutive frames from a real-world rainy video of NTURain~\cite{Chen2018RobustCNN}. From top to bottom: rainy input, 
  % MSCSC~\cite{Li2018VideoRainStreak}, 
  DRSformer~\cite{Chen2023drsformer}, S2VD~\cite{Yue2021Semi}, ESTINet~\cite{zhang2022enhanced}, MFGAN~\cite{Yang2022MFGAN}, 
  SLDNet~\cite{Yang2020Self}, 
  and ours.}
  \label{fig:realra2}
  % \vspace{-0.4cm}
\end{figure*}

==> sec_fig/result/ra3.tex <==
\begin{figure*}[t]
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/rainy/00020.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/mscsc/0020.jpg}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/sldnet/00020_res.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/drsformer/00020.png}
  
  \vspace{-2.5mm}
  \centering
  \subfloat[Rainy\label{fig:realra3-a}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/rainy/00023.jpg}}
  \hfill
  \subfloat[MSCSC~\cite{Li2018VideoRainStreak} \label{fig:realra3-b}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/mscsc/0023.jpg}}
  \hfill
  \subfloat[SLDNet~\cite{Yang2020Self} \label{fig:realra3-c}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/sldnet/00023_res.png}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer}\label{fig:realra3-d}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/drsformer/00023.png}}
  
  \vspace{1mm}
  \centering
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/s2vd/00020.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/estinet/169_0_2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/mfgan/00020_s2.png}
  \hfill
  \includegraphics[width=0.245\linewidth]{fig/result/real/ra3/ours/00020.png}
  
  \vspace{-2.5mm}
  \centering
  \subfloat[S2VD~\cite{Yue2021Semi}\label{fig:realra3-e}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/s2vd/00023.png}}
  \hfill
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:realra3-f}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/estinet/172_0_2.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:realra3-g}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/mfgan/00023_s2.png}}
  \hfill
  \subfloat[Ours\label{fig:realra3-h}]{\includegraphics[width=0.245\linewidth]{fig/result/real/ra3/ours/00023.png}}
  
    
\setlength{\abovecaptionskip}{1pt} 
\setlength{\belowcaptionskip}{-10pt}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a real-world rainy video from NTURain~\cite{Chen2018RobustCNN}. }
  \label{fig:realra3}
  \vspace{-0.4cm}
\end{figure*}

==> sec_fig/result/rainsyncomplex25.tex <==
\begin{figure*}[t]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:rainsyncomplex25-a}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/rainy/6.png}}
  \hfill
  \subfloat[MSCSC~\cite{Li2018VideoRainStreak} \label{fig:rainsyncomplex25-b}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/mscsc/0006.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:rainsyncomplex25-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/fastderain/0006.jpg}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer} \label{fig:rainsyncomplex25-d}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/drsformer/rect_1_6.png}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:rainsyncomplex25-e}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/estinet/rect_5_0_2.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:rainsyncomplex25-f}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/mfgan/rect_6.png}}
  \hfill
  \subfloat[Ours\label{fig:rainsyncomplex25-g}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/ours/rect_6.png}}
  \hfill
  \subfloat[Clean\label{fig:rainsyncomplex25-h}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsyncomplex25/gt/6.png}}
  
    
\setlength{\abovecaptionskip}{2pt} 
\setlength{\belowcaptionskip}{-10pt}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a synthetic rainy video from RainSynComplex25~\cite{Liu2018Erase}.}
  \label{fig:rainsyncomplex25}
  % \vspace{-3mm}
\end{figure*}

==> sec_fig/result/rainsynlight25.tex <==
\begin{figure*}[thp]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:rainsynlight25-a}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/rainy/6.png}}
  \hfill
  \subfloat[MSCSC~\cite{Li2018VideoRainStreak} \label{fig:rainsynlight25-b}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/mscsc/0006.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:rainsynlight25-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/fastderain/0006.jpg}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer} \label{fig:rainsynlight25-d}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/drsformer/rect_9_6.png}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:rainsynlight25-e}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/estinet/rect_239_0_2.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:rainsynlight25-f}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/mfgan/rect_6.png}}
  \hfill
  \subfloat[Ours\label{fig:rainsynlight25-g}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/ours/rect_6.png}}
  \hfill
  \subfloat[Clean\label{fig:rainsynlight25-h}]{\includegraphics[width=0.245\linewidth]{fig/result/rainsynlight25/gt/6.png}}
  
    
\setlength{\abovecaptionskip}{2pt} 
\setlength{\belowcaptionskip}{-1pt}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a synthetic rainy video from RainSynLight25~\cite{Liu2018Erase}.}
  \label{fig:rainsynlight25}
  % \vspace{-0.5cm}
\end{figure*}

==> sec_fig/result/real/forest.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_rainy_0017.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_sldnet_00017_res.png}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_drsformer_0017.png}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_drsformer_0017.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_estinet_0017.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_mfgan_00017_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_s2vd_00017.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_ours_0017.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on a real-world rainy video from Internet.}
  \label{fig:real-supple-forest}
\end{figure*}

==> sec_fig/result/real/ra2-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00049.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mscsc_0049.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_fastderain_0049.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00049.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00049.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00049_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00049.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00049.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra2-1}
\end{figure*}

==> sec_fig/result/real/ra2-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00063.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mscsc_0063.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_fastderain_0063.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00063.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00063.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00063_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainmamba_00063.png}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00063.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra2-2}
\end{figure*}

==> sec_fig/result/real/ra2-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00064.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mscsc_0064.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_fastderain_0064.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00064.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00064.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00064_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainmamba_00064.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00064.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra2-3}
\end{figure*}

==> sec_fig/result/real/ra2-4.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00065.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mscsc_0065.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_fastderain_0065.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00065.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00065.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00065_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainmamba_00065.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00065.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra2-4}
\end{figure*}

==> sec_fig/result/real/ra2.tex <==
\begin{figure*}
  \centering
  \subfloat[Rainy\label{fig:ra2-2-a}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00049.jpg}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_patch0_00049.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00063.jpg}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_patch0_00063.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00064.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_rainy_patch0_00064.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_rainy_patch1_00064.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_rainy_00065.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_rainy_patch0_00065.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_rainy_patch1_00065.jpg}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[DRSformer.~\cite{Chen2023drsformer}\label{fig:ra2-2-c}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00049.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_patch0_00049.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00063.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_patch0_00063.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00064.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_drsformer_patch0_00064.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_drsformer_patch1_00064.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_drsformer_00065.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_drsformer_patch0_00065.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_drsformer_patch1_00065.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[S2VD~\cite{Yue2021Semi}\label{fig:ra2-2-d}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_00049.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_patch0_00049.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_00063.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_patch0_00063.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_00064.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_s2vd_patch0_00064.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_s2vd_patch1_00064.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_s2vd_00065.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_s2vd_patch0_00065.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_s2vd_patch1_00065.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[ESTINet~\cite{zhang2022enhanced}\label{fig:ra2-2-e}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00049.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_patch0_00049.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00063.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_patch0_00063.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00064.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_estinet_patch0_00064.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_estinet_patch1_00064.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_estinet_00065.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_estinet_patch0_00065.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_estinet_patch1_00065.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:ra2-2-f}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00049_s2.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_patch0_00049_s2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00063_s2.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_patch0_00063_s2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00064_s2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_mfgan_patch0_00064_s2.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_mfgan_patch1_00064_s2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_mfgan_00065_s2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_mfgan_patch0_00065_s2.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_mfgan_patch1_00065_s2.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[SLDNet~\cite{Yang2020Self}\label{fig:ra2-2-b}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_00049_res.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_patch0_00049_res.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_00063_res.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_patch0_00063_res.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_00064_res.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_sldnet_patch0_00064_res.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_sldnet_patch1_00064_res.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_sldnet_00065_res.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_sldnet_patch0_00065_res.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_sldnet_patch1_00065_res.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[Ours\label{fig:ra2-2-g}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00049.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_patch0_00049.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00063.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_patch0_00063.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00064.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_ours_patch0_00064.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_ours_patch1_00064.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra2/ra2_ours_00065.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_ours_patch0_00065.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra2/ra2_ours_patch1_00065.png}
    \end{minipage}
    }
    \vspace{-1mm}
  \caption{The visual comparison among the state-of-the-art deraining methods on four consecutive frames from a real-world rainy video of NTURain~\cite{Chen2018RobustCNN}. }
  \label{fig:realra2}
  \vspace{-2mm}
\end{figure*}

==> sec_fig/result/real/ra3-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainy_00020.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mscsc_0020.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_fastderain_0020.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_drsformer_00020.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_estinet_169_0_2.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mfgan_00020_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainmamba_00020.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_ours_00020.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra3-1}
\end{figure*}

==> sec_fig/result/real/ra3-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainy_00023.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mscsc_0023.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_fastderain_0023.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_drsformer_00023.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_estinet_172_0_2.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mfgan_00023_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainmamba_00023.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_ours_00023.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra3-2}
\end{figure*}

==> sec_fig/result/real/ra3.tex <==
\begin{figure*}
  \centering
  \subfloat[Rainy\label{fig:ra3-2-a}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainy_00020.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_rainy_patch0_00020.jpg}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_rainy_patch1_00020.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_rainy_00023.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_rainy_patch0_00023.jpg}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_rainy_patch1_00023.jpg}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[DRSformer.~\cite{Chen2023drsformer}\label{fig:ra3-2-c}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_drsformer_00020.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_drsformer_patch0_00020.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_drsformer_patch1_00020.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_drsformer_00023.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_drsformer_patch0_00023.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_drsformer_patch1_00023.png}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[S2VD~\cite{Yue2021Semi}\label{fig:ra3-2-d}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_s2vd_00020.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_s2vd_patch0_00020.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_s2vd_patch1_00020.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_s2vd_00023.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_s2vd_patch0_00023.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_s2vd_patch1_00023.png}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[ESTINet~\cite{zhang2022enhanced}\label{fig:ra3-2-e}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_estinet_169_0_2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_estinet_patch0_169_0_2.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_estinet_patch1_169_0_2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_estinet_172_0_2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_estinet_patch0_172_0_2.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_estinet_patch1_172_0_2.png}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:ra3-2-f}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mfgan_00020_s2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_mfgan_patch0_00020_s2.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_mfgan_patch1_00020_s2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_mfgan_00023_s2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_mfgan_patch0_00023_s2.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_mfgan_patch1_00023_s2.png}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[SLDNet~\cite{Yang2020Self}\label{fig:ra3-2-b}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_sldnet_00020_res.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_sldnet_patch0_00020_res.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_sldnet_patch1_00020_res.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_sldnet_00023_res.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_sldnet_patch0_00023_res.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_sldnet_patch1_00023_res.png}
    \end{minipage}
    }
    \hspace{-2.4mm}
    \subfloat[Ours\label{fig:ra3-2-g}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_ours_00020.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_ours_patch0_00020.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_ours_patch1_00020.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra3/ra3_ours_00023.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_ours_patch0_00023.png}
    \hspace{-1.3mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/ra3/ra3_ours_patch1_00023.png}
    \end{minipage}
    }
    \vspace{-1mm}
  \caption{The qualitative comparison among ours and the state-of-the-art methods on a real-world rainy video from NTURain~\cite{Chen2018RobustCNN}. }
  \label{fig:realra3}
  \vspace{-2mm}
\end{figure*}

==> sec_fig/result/real/ra4-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_rainy_00066.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_mscsc_0066.jpg}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_fastderain_0066.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_drsformer_00066.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_estinet_00066.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_mfgan_66.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_rainmamba_00066.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_ours_00066.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on NTURain~\cite{Chen2018RobustCNN}.}
  \label{fig:real-supple-ra4-1}
\end{figure*}

==> sec_fig/result/real/real.tex <==
\begin{figure*}
  \centering
  \subfloat[Rainy\label{fig:realother-2-a}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_rainy_00066.jpg}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_rainy_patch0_00066.jpg}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_rainy_0052.jpeg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_rainy_patch0_0052.jpeg}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_rainy_patch1_0052.jpeg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_rainy_0017.jpg}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_rainy_patch0_0017.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_rainy_00022.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_rainy_patch0_00022.jpg}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_rainy_patch1_00022.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_rainy_00026.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_rainy_patch0_00026.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_rainy_patch1_00026.jpg}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_rainy_00031.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_rainy_patch0_00031.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_rainy_patch1_00031.jpg}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[DRSformer.~\cite{Chen2023drsformer}\label{fig:realother-2-c}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_drsformer_00066.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_drsformer_patch0_00066.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_drsformer_0052.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_drsformer_patch0_0052.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_drsformer_patch1_0052.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_drsformer_0017.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_drsformer_patch0_0017.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_drsformer_00022.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_drsformer_patch0_00022.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_drsformer_patch1_00022.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_drsformer_00026.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_drsformer_patch0_00026.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_drsformer_patch1_00026.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_drsformer_00031.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_drsformer_patch0_00031.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_drsformer_patch1_00031.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[S2VD~\cite{Yue2021Semi}\label{fig:realother-2-d}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_s2vd_00066.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_s2vd_patch0_00066.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_s2vd_00052.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_s2vd_patch0_00052.jpg}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_s2vd_patch1_00052.jpg}

    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_s2vd_00017.jpg}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_s2vd_patch0_00017.jpg}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_s2vd_00022.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_s2vd_patch0_00022.jpg}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_s2vd_patch1_00022.jpg}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_s2vd_00026.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_s2vd_patch0_00026.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_s2vd_patch1_00026.jpg}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_s2vd_00031.jpg}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_s2vd_patch0_00031.jpg}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_s2vd_patch1_00031.jpg}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[ESTINet~\cite{zhang2022enhanced}\label{fig:realother-2-e}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_estinet_00066.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_estinet_patch0_00066.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_estinet_0052.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_estinet_patch0_0052.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_estinet_patch1_0052.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_estinet_0017.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_estinet_patch0_0017.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_estinet_00022.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_estinet_patch0_00022.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_estinet_patch1_00022.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_estinet_00026.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_estinet_patch0_00026.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_estinet_patch1_00026.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_estinet_00031.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_estinet_patch0_00031.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_estinet_patch1_00031.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:realother-2-f}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_mfgan_66.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_mfgan_patch0_66.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_mfgan_00052_s2.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_mfgan_patch0_00052_s2.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_mfgan_patch1_00052_s2.png}

    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_mfgan_00017_s2.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_mfgan_patch0_00017_s2.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_mfgan_00022.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_mfgan_patch0_00022.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_mfgan_patch1_00022.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_mfgan_00026.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_mfgan_patch0_00026.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_mfgan_patch1_00026.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_mfgan_00031.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_mfgan_patch0_00031.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_mfgan_patch1_00031.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[SLDNet~\cite{Yang2020Self}\label{fig:realother-2-b}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_sldnet_00066_res.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_sldnet_patch0_00066_res.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_sldnet_00052_res.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_sldnet_patch0_00052_res.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_sldnet_patch1_00052_res.png}

    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_sldnet_00017_res.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_sldnet_patch0_00017_res.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_sldnet_00022.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_sldnet_patch0_00022.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_sldnet_patch1_00022.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_sldnet_00026.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_sldnet_patch0_00026.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_sldnet_patch1_00026.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_sldnet_00031.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_sldnet_patch0_00031.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_sldnet_patch1_00031.png}
    \end{minipage}
    }
    \hspace{-3.4mm}
    \subfloat[Ours\label{fig:realother-2-g}]{
  \begin{minipage}{0.1389\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_ours_00066.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/ra4/ra4_ours_patch0_00066.png}
    
    \centering
    \includegraphics[trim=0 120mm 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_ours_0052.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_ours_patch0_0052.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/yard/yard_ours_patch1_0052.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_ours_0017.png}
    \hspace{-0mm}
    \includegraphics[width=1\linewidth]{fig/result/real/forest/forest_ours_patch0_0017.png}
    
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_ours_00022.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_ours_patch0_00022.png}
    \hspace{-2mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_22/rrodt_22_ours_patch1_00022.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_ours_00026.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_ours_patch0_00026.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_39/rrodt_39_ours_patch1_00026.png}
     
    \centering
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_ours_00031.png}
    \hspace{-0mm}
    \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_ours_patch0_00031.png}
    \hspace{-2mm}
     \includegraphics[width=0.490\linewidth]{fig/result/real/rrodt_55/rrodt_55_ours_patch1_00031.png}
    \end{minipage}
    }
    \vspace{-1mm}
  \caption{The visual comparison among the state-of-the-art deraining methods on four sample frames from real-world rainy videos of \cite{Chen2018RobustCNN}, \cite{Li2018VideoRainStreak}, \cite{Yang2019Frame}, and our RRODT. }
  \label{fig:realother}
  \vspace{-2mm}
\end{figure*}

==> sec_fig/result/real/rrodt-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_rainy_00022.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_sldnet_00022.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_fastderain_00022.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_drsformer_00022.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_estinet_00022.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_mfgan_00022.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_rainmamba_00022.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_22/rrodt_22_ours_00022.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on RVDT.}
  \label{fig:real-supple-rrodt-1}
\end{figure*}

==> sec_fig/result/real/rrodt-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_rainy_00026.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_sldnet_00026.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_fastderain_00026.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_drsformer_00026.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_estinet_00026.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_mfgan_00026.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_rainmamba_00026.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_39/rrodt_39_ours_00026.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on RVDT.}
  \label{fig:real-supple-rrodt-2}
\end{figure*}

==> sec_fig/result/real/rrodt-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_rainy_00031.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_sldnet_00031.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_fastderain_00031.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_drsformer_00031.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_estinet_00031.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_mfgan_00031.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_rainmamba_00031.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_55/rrodt_55_ours_00031.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on RVDT.}
  \label{fig:real-supple-rrodt-3}
\end{figure*}

==> sec_fig/result/real/rrodt-4.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_rainy_00020.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_sldnet_00020.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_fastderain_00020.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_drsformer_00020.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_estinet_00020.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_ours_00020.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_rainmamba_00020.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/real/rrodt_56/rrodt_56_mfgan_00020.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on RVDT.}
  \label{fig:real-supple-rrodt-4}
\end{figure*}

==> sec_fig/result/real/yard.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_rainy_0052.jpeg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_sldnet_00052_res.png}
  \end{subfigure}
    \subcaption[]{MSCSC~\cite{Jiang2020MultiScale}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_drsformer_0052.png}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_drsformer_0052.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_estinet_0052.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_mfgan_00052_s2.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_s2vd_00052.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 365 0 0,clip,width=1\linewidth]{fig/result/real/yard/yard_ours_0052.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world video deraining on a real-world rainy video from Internet.}
  \label{fig:real-supple-yard}
\end{figure*}

==> sec_fig/result/rrodt_gtr-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/rainy/00053.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/sldnet/00053.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/fastderain/00053.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/drsformer/00053.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/estinet/00053.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/mfgan/00053.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/s2vd/00053.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/ours/00053.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object tracking on RVDT using GTR~\cite{zhou2022gtr}.}
  \label{fig:real-supple-gtr-1}
\end{figure*}

==> sec_fig/result/rrodt_gtr-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/rainy/00076.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/sldnet/00076.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/fastderain/00076.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/drsformer/00076.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/estinet/00076.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/mfgan/00076.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/s2vd/00076.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/ours/00076.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object tracking on RVDT using GTR~\cite{zhou2022gtr}.}
  \label{fig:real-supple-gtr-2}
\end{figure*}

==> sec_fig/result/rrodt_gtr-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/rainy/00089.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/sldnet/00089.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/fastderain/00089.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/drsformer/00089.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/estinet/00089.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/mfgan/00089.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/s2vd/00089.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/ours/00089.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object tracking on RVDT using GTR~\cite{zhou2022gtr}.}
  \label{fig:real-supple-gtr-3}
\end{figure*}

==> sec_fig/result/rrodt_gtr-4.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/rainy/00110.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/sldnet/00110.png}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/fastderain/00110.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/drsformer/00110.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/estinet/00110.png}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/mfgan/00110.png}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/s2vd/00110.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/gtr/ours/00110.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object tracking on RVDT using GTR~\cite{zhou2022gtr}.}
  \label{fig:real-supple-gtr-4}
\end{figure*}

==> sec_fig/result/rrodt_gtr.tex <==
\begin{figure*}[t]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:rrodt_gtr-a}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/rainy/00110.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:rrodt_gtr-b}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/fastderain/00110.jpg}}
  \hfill
  \subfloat[SLDNet~\cite{Yang2020Self} \label{fig:rrodt_gtr-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/sldnet/00110.png}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer} \label{fig:rrodt_gtr-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/drsformer/00110.png}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[S2VD~\cite{Yue2021Semi} \label{fig:rrodt_gtr-d}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/s2vd/00110.jpg}}
  \hfill
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:rrodt_gtr-e}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/estinet/00110.png}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:rrodt_gtr-f}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/mfgan/00110.png}}
  \hfill
  \subfloat[Ours\label{fig:rrodt_gtr-g}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/gtr/ours/00110.png}}
  
    
\setlength{\abovecaptionskip}{1pt} 
\setlength{\belowcaptionskip}{-10pt}
  \caption{A deraining and object tracking result by GTR~\cite{zhou2022gtr} on our RRODT.}
  \label{fig:rrodt_gtr}
  % \vspace{-0.6cm}
\end{figure*}

==> sec_fig/result/rrodt_mega-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/rainy/00129.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/sldnet/00129.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/fastderain/00129.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/drsformer/00129.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/estinet/00129.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/mfgan/00129.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/s2vd/00129.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/ours/00129.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using mega~\cite{Chen2020MEGA}.}
  \label{fig:real-supple-mega-1}
\end{figure*}

==> sec_fig/result/rrodt_mega-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/rainy/00163.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/sldnet/00163.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/fastderain/00163.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/drsformer/00163.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/estinet/00163.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/mfgan/00163.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/s2vd/00163.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/ours/00163.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using mega~\cite{Chen2020MEGA}.}
  \label{fig:real-supple-mega-2}
\end{figure*}

==> sec_fig/result/rrodt_mega-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/rainy/00193.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/sldnet/00193.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/fastderain/00193.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/drsformer/00193.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/estinet/00193.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/mfgan/00193.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/s2vd/00193.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/mega/ours/00193.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using mega~\cite{Chen2020MEGA}.}
  \label{fig:real-supple-mega-3}
\end{figure*}

==> sec_fig/result/rrodt_mega.tex <==
\begin{figure*}[t]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:rrodt_mega-a}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/rainy/00129_cu.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:rrodt_mega-b}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/fastderain/00129_cu.jpg}}
  \hfill
  \subfloat[SLDNet~\cite{Yang2020Self} \label{fig:rrodt_mega-c}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/sldnet/00129_cu.jpg}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer} \label{fig:rrodt_mega-c}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/drsformer/00129_cu.jpg}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[S2VD~\cite{Yue2021Semi} \label{fig:rrodt_mega-d}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/s2vd/00129_cu.jpg}}
  \hfill
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:rrodt_mega-e}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/estinet/00129_cu.jpg}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:rrodt_mega-f}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/mfgan/00129_cu.jpg}}
  \hfill
  \subfloat[Ours\label{fig:rrodt_mega-g}]{\includegraphics[trim={2.3cm 0 0 2.3cm},clip,width=0.245\linewidth]{fig/result/rrodt/mega/ours/00129_cu.jpg}}
  
    
\setlength{\abovecaptionskip}{1pt} 
\setlength{\belowcaptionskip}{-1pt}
  \caption{A deraining and detection result by MEGA~\cite{Chen2020MEGA} on our RRODT. All existing methods cannot avoid the detector from predicting two cars by mistake, while only ours yields the most satisfactory result.}
  \label{fig:rrodt_mega}
  \vspace{-0.4cm}
\end{figure*}

==> sec_fig/result/rrodt_yolov3-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/rainy/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/sldnet/det_00028_res.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/fastderain/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/drsformer/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/estinet/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/mfgan/det_28.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/s2vd/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/ours/det_00028.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using YOLOv3~\cite{redmon2018yolov3}.}
  \label{fig:real-supple-yolov3-1}
\end{figure*}

==> sec_fig/result/rrodt_yolov3-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/rainy/det_00060.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/sldnet/det_00060_res.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/fastderain/det_00060.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/drsformer/det_00060.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/estinet/det_00060.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/mfgan/det_60.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/s2vd/det_00060_cu.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/ours/det_00060.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using YOLOv3~\cite{redmon2018yolov3}.}
  \label{fig:real-supple-yolov3-2}
\end{figure*}

==> sec_fig/result/rrodt_yolov3-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/rainy/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/sldnet/det_00137_res.jpg}
  \end{subfigure}
    \subcaption[]{SLDNet~\cite{Yang2020Self}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/fastderain/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{FastDerain~\cite{Jiang2019FastDerain}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/drsformer/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/estinet/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{ESTINet~\cite{zhang2022enhanced}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/mfgan/det_137.jpg}
  \end{subfigure}
    \subcaption[]{MFGAN~\cite{Yang2022MFGAN}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/s2vd/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{RainMamba~\cite{wu2024rainmamba}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.405\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rrodt/yolov3/ours/det_00137.jpg}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of object detection on RVDT using YOLOv3~\cite{redmon2018yolov3}.}
  \label{fig:real-supple-yolov3-3}
\end{figure*}

==> sec_fig/result/rrodt_yolov3.tex <==
\begin{figure*}[t]
\scriptsize
\captionsetup{font={small}}
% \setlength{\abovecaptionskip}{-5pt} 
  \centering
  \subfloat[Rainy\label{fig:rrodt_yolov3-a}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/rainy/det_00060_cu.jpg}}
  \hfill
  \subfloat[FastDeRain~\cite{Jiang2019FastDerain} \label{fig:rrodt_yolov3-b}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/fastderain/det_00060_cu.jpg}}
  \hfill
  \subfloat[SLDNet~\cite{Yang2020Self} \label{fig:rrodt_yolov3-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/sldnet/det_00060_cu.jpg}}
  \hfill
  \subfloat[DRSformer~\cite{Chen2023drsformer} \label{fig:rrodt_yolov3-c}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/drsformer/det_00060_cu.jpg}}
  
  % \vspace{-2.5mm}
  \centering
  \subfloat[S2VD~\cite{Yue2021Semi} \label{fig:rrodt_yolov3-d}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/s2vd/det_00060_cu.jpg}}
  \hfill
  \subfloat[ESTINet~\cite{zhang2022enhanced} \label{fig:rrodt_yolov3-e}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/estinet/det_00060_cu.jpg}}
  \hfill
  \subfloat[MFGAN~\cite{Yang2022MFGAN}\label{fig:rrodt_yolov3-f}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/mfgan/det_00060_cu.jpg}}
  \hfill
  \subfloat[Ours\label{fig:rrodt_yolov3-g}]{\includegraphics[width=0.245\linewidth]{fig/result/rrodt/yolov3/ours/det_00060_cu.jpg}}
  
    
\setlength{\abovecaptionskip}{1pt} 
\setlength{\belowcaptionskip}{-10pt}
  \caption{A deraining and detection result by YOLO-v3~\cite{redmon2018yolov3} on our RRODT. DRSformer~\cite{Chen2023drsformer}, S2VD~\cite{Yue2021Semi} and ESTINet~\cite{zhang2022enhanced} cannot help the detector recognize the car. FastDeRain~\cite{Jiang2019FastDerain} and SLDNet~\cite{Yang2020Self} make the detector confused between ``car'' and ``train''. The detected box on the derained frame by MFGAN~\cite{Yang2022MFGAN} is inaccurate, while only ours yields the most satisfactory result.}
  \label{fig:rrodt_yolov3}
  \vspace{-5mm}
\end{figure*}

==> sec_fig/result/single_image_deraining.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.310\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 91 0 0,clip,width=1\linewidth]{fig/result/single/rainy/5.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 60 0 0,clip,width=1\linewidth]{fig/result/single/rainy/6.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 90 0 0,clip,width=1\linewidth]{fig/result/single/rainy/12.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 50 0 0,clip,width=1\linewidth]{fig/result/single/rainy/14.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/single/rainy/54.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.310\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 91 0 0,clip,width=1\linewidth]{fig/result/single/drsformer/5.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 60 0 0,clip,width=1\linewidth]{fig/result/single/drsformer/6.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 90 0 0,clip,width=1\linewidth]{fig/result/single/drsformer/12.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 50 0 0,clip,width=1\linewidth]{fig/result/single/drsformer/14.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/single/drsformer/54.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{Chen2023drsformer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.310\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 91 0 0,clip,width=1\linewidth]{fig/result/single/ours/5.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 60 0 0,clip,width=1\linewidth]{fig/result/single/ours/6.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 90 0 0,clip,width=1\linewidth]{fig/result/single/ours/12.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 50 0 0,clip,width=1\linewidth]{fig/result/single/ours/14.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/single/ours/54.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{Visual comparisons of real-world single image deraining on Internet-Data~\cite{Wang2019Spatial}.
  The results of ours are generated by our VDMamba-single.}
  \label{fig:real-supple-single}
\end{figure*}

==> sec_fig/rrodt_example.tex <==

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/54/00004.jpg}
  \hfill
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/54/00005.jpg}
  \hfill
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/54/00006.jpg}

  \vspace{1mm}
  \centering
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/56/00024.jpg}
  \hfill
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/56/00025.jpg}
  \hfill
  \includegraphics[width=0.324\linewidth]{fig/rrodt_example/56/00026.jpg}
  % \vspace{1mm}
  % \centering
  % \includegraphics[width=0.324\linewidth]{fig/rrodt_example/55/00025.jpg}
  % \hfill
  % \includegraphics[width=0.324\linewidth]{fig/rrodt_example/55/00026.jpg}
  % \hfill
  % \includegraphics[width=0.324\linewidth]{fig/rrodt_example/55/00027.jpg}
\setlength{\abovecaptionskip}{-7pt} 
\setlength{\belowcaptionskip}{-7pt}
  \caption{Example frames of real-world rainy sequences in RVDT.}
  \label{fig:rrodt_example}
  \vspace{-2mm}
\end{figure}

==> sec_fig/rvdt_example.tex <==

\begin{figure}[tp]
  \centering
  % \includegraphics[width=0.24\linewidth]{fig/rrodt_example/54/00004.jpg}
  % \hfill
    \begin{annotationimage}{width=0.24\linewidth}{fig/rrodt_example/54/00005.jpg}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Frame 1 of video 1};
    \end{annotationimage}
  \hspace{-2mm}
    \begin{annotationimage}{width=0.24\linewidth}{fig/rrodt_example/54/00006.jpg}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Frame 2 of video 1};
    \end{annotationimage}
  \hspace{-2mm}
    \begin{annotationimage}{width=0.24\linewidth}{fig/rrodt_example/56/00024.jpg}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Frame 1 of video 2};
    \end{annotationimage}
  \hspace{-2mm}
    \begin{annotationimage}{width=0.24\linewidth}{fig/rrodt_example/56/00025.jpg}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Frame 2 of video 2};
    \end{annotationimage}
  % \hfill
  % \includegraphics[width=0.24\linewidth]{fig/rrodt_example/56/00026.jpg}
  % \vspace{1mm}
  % \centering
  % \includegraphics[width=0.24\linewidth]{fig/rrodt_example/55/00025.jpg}
  % \hfill
  % \includegraphics[width=0.24\linewidth]{fig/rrodt_example/55/00026.jpg}
  % \hfill
  % \includegraphics[width=0.24\linewidth]{fig/rrodt_example/55/00027.jpg}
  \vspace{-3mm}
  \caption{4 sample frames of real-world rainy sequences in RVDT.}
  \label{fig:rrodt_example}
  \vspace{-6mm}
\end{figure}

==> sec_tab/niqe.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\footnotesize
\renewcommand\arraystretch{0.9}
\tabcolsep=1.4mm
  \centering
  \caption{The metrics comparison of real-world rain streak removal for non-reference quality assessment on the real videos of NTURain~\cite{Chen2018RobustCNN}.}
  % \vspace{-3mm}
    \begin{tabular}{lrrrrrrrr}
    \toprule
          & Input &  FastDerain~\cite{Jiang2019FastDerain} & S2VD~\cite{Yue2021Semi} & ESTINet~\cite{zhang2022enhanced} & MFGAN~\cite{Yang2022MFGAN} & RainMamba~\cite{wu2024rainmamba} & Ours \\
    \midrule
    NIQE$\downarrow$ & 3.32  & 4.47  & 4.51  & 4.49  & 4.33  & 4.45  & \textbf{2.94} \\
    BRISQUE$\downarrow$ & 20.21 & 21.49 & 22.87 & 23.43 & 22.39 & 22.69 & \textbf{16.81} \\
    \bottomrule
    \end{tabular}%
  \label{tab:niqe}%
  % \vspace{-4mm}
\end{table}%


==> sec_tab/nturain.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\footnotesize
\renewcommand{\arraystretch}{1.}
\setlength{\tabcolsep}{0.85mm}
  \centering
  \caption{Quantitative results of various video deraining methods on the benchmark of long videos, \textit{NTURain}.}
  \vspace{-2mm}
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \hline
    \multirow{1}[4]{*}{Video} & \multicolumn{2}{c|}{Rainy}  & \multicolumn{2}{c|}{FastDeRain~\cite{Jiang2019FastDerain}} & \multicolumn{2}{c|}{SpacCNN~\cite{Chen2018RobustCNN}} & \multicolumn{2}{c|}{SLDNet~\cite{Yang2020Self}} & \multicolumn{2}{c|}{S2VD~\cite{Yue2021Semi}} & \multicolumn{2}{c|}{ESTINet~\cite{zhang2022enhanced}} & \multicolumn{2}{c|}{MFGAN~\cite{Yang2022MFGAN}} &\multicolumn{2}{c|}{RainMamba~\cite{wu2024rainmamba}} & \multicolumn{2}{c}{Ours} \\
\cline{2-19}          & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM  & PSNR  & SSIM \\
    \hline
    a1    & 29.71  & 0.9149   & 29.29  & 0.9159  & 30.57  & 0.9334  & 33.72  & 0.9508  & 36.39  & 0.9658  & 36.99  & 0.9698  & 37.27  & 0.9702 & 38.29  & 0.9834   & \textbf{38.82 } & \textbf{0.9756} \\
    a2    & 29.30  & 0.9284   & 30.21  & 0.9245  & 31.29  & 0.9356  & 33.82  & 0.9512  & 33.06  & 0.9519  & 34.48  & 0.9611  & 35.55  & 0.9620  & 34.56 & 0.9741 & \textbf{37.45 } & \textbf{0.9699} \\
    a3    & 29.08  & 0.8964  & 29.94  & 0.9039  & 30.63  & 0.9247  & 33.12  & 0.9404  & 35.75  & 0.9564  & 36.09  & 0.9649  & 36.44  & 0.9631 & 36.44 & 0.9765 & \textbf{38.20 } & \textbf{0.9711} \\
    a4    & 32.62  & 0.9381 & 34.69  & 0.9707  & 35.30  & 0.9620  & 37.35  & 0.9722  & 39.53  & 0.9779  & 40.00  & 0.9795  & 41.15  & 0.9851 & 41.48 &  0.9884 & \textbf{42.09 } & \textbf{0.9871} \\
    \hline
    b1    & 30.03  & 0.8956  & 29.35  & 0.9139  & 32.26  & 0.9454  & 34.21  & 0.9482  & 37.34  & 0.9712  & 37.15  & 0.9683  & 38.82  & 0.9778 & 39.27 & 0.9828 & \textbf{39.77 } & \textbf{0.9799} \\
    b2    & 30.69  & 0.8874  & 31.90  & 0.9520  & 35.11  & 0.9677  & 35.80  & 0.9595  & 40.55  & 0.9821  & 40.01  & 0.9752  & 40.42  & 0.9843 & 41.36 & 0.9855  & \textbf{40.96 } & \textbf{0.9850} \\
    b3    & 32.31  & 0.9299  & 29.28  & 0.9287  & 34.69  & 0.9566  & 36.34  & 0.9614  & 38.83  & 0.9754  & 38.06  & 0.9740  & 41.13  & 0.9858 & 40.81 & 0.9867 & \textbf{41.86 } & \textbf{0.9865} \\
    b4    & 29.41  & 0.8933  & 27.70  & 0.9095  & 34.87  & 0.9536  & 33.85  & 0.9469  & 37.53  & 0.9657  & 36.81  & 0.9653  & 40.43 & \textbf{0.9823 } & 41.24 & 0.9856 & \textbf{40.83 } & 0.9821 \\
    \hline
    Mean  & 30.41  & 0.9108   & 30.30  & 0.9274  & 33.11  & 0.9475  & 34.89  & 0.9540  & 37.37  & 0.9683  & 37.48  & 0.9700  & 38.92  & 0.9764 & 37.87 &  0.9738   & \textbf{40.00 } & \textbf{0.9796} \\
    \hline
    \end{tabular}%
  \label{tab:nturain}%
  % \vspace{-6mm}
\end{table*}%


==> sec_tab/rrodt_stats.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[tp]
\renewcommand{\arraystretch}{.8}
\footnotesize
  \centering
  \caption{The statistics of the proposed RVDT.}
  \vspace{-3mm}
    \begin{tabular}{ccc|ccc}
    \toprule
    Class & Count & Unique & Class & Count & Unique\\
    \midrule
    car   & 11180 & 167 & handbag & 350 & 1\\
    person & 9505 & 99 & bus   & 283 & 5\\
    motorbike & 5931 & 76 & aeroplane & 229 & 1\\
    umbrella & 2840 & 24 & traffic light & 148 & 4\\
    truck & 1269 & 14 & boat  & 130 & 1\\
    cow   & 573 & 8 & backpack & 122 & 2\\
    bicycle & 402 & 5  & train & 115 & 1\\
    \bottomrule
    \end{tabular}%
    % \begin{tabular}{cccc}
    % \toprule
    % Class & Count & Class & Count \\
    % \midrule
    % car   & 11180 & handbag & 350 \\
    % person & 9505  & bus   & 283 \\
    % motorbike & 5931  & aeroplane & 229 \\
    % umbrella & 2840  & traffic light & 148 \\
    % truck & 1269  & boat  & 130 \\
    % cow   & 573   & backpack & 122 \\
    % bicycle & 402   & train & 115 \\
    % \bottomrule
    % \end{tabular}%
  \label{tab:rrodt_stats}%
  \vspace{-3mm}
\end{table}%


==> sec_tab/table_rebuttal.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[tp]
\footnotesize
  \centering
  % \tabcolsep=1.5mm
  \renewcommand\arraystretch{.8}
  \caption{Further comparisons of SLDNet and S2VD on NTURain}
  \vspace{-3mm}
    \begin{tabular}{cccc}
    \toprule
          & SLDNet & S2VD  & Ours \\
    \midrule
    PSNR/SSIM & 34.89/0.9540 & 37.37/0.9683 & \textbf{39.74/0.9791} \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab_rebuttal_a}%
  \vspace{-2mm}
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[tp]
\footnotesize
  \centering
  \tabcolsep=1.3mm
  \renewcommand\arraystretch{.8}
  \caption{Further comparisons of SpacCNN and J4RNet on RVDT}
  \vspace{-3mm}
    \begin{tabular}{cccc}
    \toprule
          & SpacCNN & J4RNet & Ours \\
    \midrule
    mAP1/mAP2 & 41.33/42.26 & 39.01/43.81 & \textbf{42.51/46.27} \\
    IDF1/MOTA/MOTP & 66.5/30.4/20.4 & 66.9/28.9/20.3 & \textbf{68.3/31.8/21.2} \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab_rebuttal_b}%
  \vspace{-2mm}
\end{table}%

